Small-x Processes in Perturbative Quantum Chromodynamics

Starting from a rewiev of DGLAP and BFKL evolution equations for small-x processes, a sistematic study is performed in order to understand the limits of both the formulations and to improve them in a unique framework, which aims to cover the whole range of applicability of perturbative QCD and which describes the transition mechanism from perturbative to non-perturbative physics in the region where unitarity contributions are expected not to be important.

==> overline.tex <==
\catcode`\@=11 % This allows us to modify PLAIN macros.
%\def\@oddhead{\underline{\makebox[\hsize]{{\rightmark}\hfill{\thepage}}}}% Right heading.
%\def\@evenhead{\underline{\makebox[\hsize]{{\thepage}\hfill{\leftmark}}}}% Left heading.
\def\@oddhead{\underline{\makebox[\hsize]{\null\hfill\thepage}}}% Right heading.
\def\@evenhead{\underline{\makebox[\hsize]{\thepage\hfill\null}}}% Left heading.

